Combating Spatial Disorientation in a Dynamic Self-Stabilization Task Using AI Assistants

Spatial disorientation is a leading cause of fatal aircraft accidents. This paper explores the potential of AI agents to aid pilots in maintaining balance and preventing unrecoverable losses of control by offering cues and corrective measures that ameliorate spatial disorientation. A multi-axis rotation system (MARS) was used to gather data from human subjects self-balancing in a spaceflight analog condition. We trained models over this data to create "digital twins" that exemplified performance characteristics of humans with different proficiency levels. We then trained various reinforcement learning and deep learning models to offer corrective cues if loss of control is predicted. Digital twins and assistant models then co-performed a virtual inverted pendulum (VIP) programmed with identical physics. From these simulations, we picked the 5 best-performing assistants based on task metrics such as crash frequency and mean distance from the direction of balance. These were used in a co-performance study with 20 new human subjects performing a version of the VIP task with degraded spatial information. We show that certain AI assistants were able to improve human performance and that reinforcement-learning based assistants were objectively more effective but rated as less trusted and preferable by humans.

==> assts_table.tex <==
\begin{table*}[h!]
\centering
 \resizebox{\textwidth}{!}{
 \begin{tabular}{lcccccccc}
\toprule
        {\bf Assistant} & {\bf Crashes}$\downarrow$  & {\bf \% destab.}$\downarrow$   & {\bf $\mu\lvert\theta\rvert$ ($^\circ$)}$\downarrow$ & {\bf $\sigma(\theta)$ ($^\circ$)}$\downarrow$ & {\bf $\mu\lvert Mag\rvert_{vel}$ ($^\circ$/s)}$\downarrow$ & {\bf $\sigma(\lvert Mag\rvert_{vel})$ ($^\circ$/s)}$\downarrow$ & {\bf $vel$ RMS}$\downarrow$         & {\bf $\mu\lvert d\rvert$}$\downarrow$ \\
\midrule
SAC             & \small 0 & \small 27.2 & \small 9.8 & \small 2.4 & \small 9.7 & \small 12.3 & \small 12.3 & \small .52\\
\midrule
SAC-BC          & \small 0 & \small 0.0 & \small 2.4 & \small 3.2 & \small 5.8 & \small 7.8 & \small 7.9 & \small .03 \\
\midrule
SAC-AIRL        & \small 0 & \small 12.2 & \small 7.7 & \small 0.7 & \small 1.0 & \small 1.3 & \small 1.3 & \small .08 \\
\midrule
DDPG            & \small 0 & \small 0.3 & \small 5.3 & \small 1.7 & \small 3.0 & \small 14.8 & \small 15.0 & \small .07 \\
\midrule
DDPG-BC         & \small 0 & \small 0.7 & \small 2.5 & \small 3.2 & \small 6.3 & \small 8.0 & \small 8.1 & \small .03 \\
\midrule
MLP-G-0         & \small 0 & \small 13.5 & \small 4.4 & \small 4.3 & \small 4.4 & \small 5.2 & \small 5.6 & \small .05 \\
\midrule
MLP-G-0.5       & \small 23 & \small 76.0 & \small 20.6 & \small 23.0 & \small 57.9 & \small 77.5 & \small 81.8 & \small .13 \\
\midrule
MLP-G-0.2       & \small 6 & \small 22.8 & \small 11.9 & \small 15.9 & \small 45.5 & \small 61.4 & \small 61.7 & \small .24 \\
\midrule
MLP-G-0.3       & \small 0 & \small 20.4 & \small 22.6 & \small 25.6 & \small 58.5 & \small 68.6 & \small 68.8 & \small .47 \\
\midrule
MLP-GM-0        & \small 0 & \small 0.0 & \small 9.7 & \small 0.2  & \small 0.3 & \small 0.7 & \small 0.7 & \small .06 \\
\midrule
MLP-GMB-0       & \small 0 & \small 20.9 & \small 4.4 & \small 4.3 & \small 4.4 & \small 5.2 & \small 5.6 & \small .05 \\
\midrule
RNN-G-0.5       & \small 7 & \small 9.6 & \small 17.2 & \small 21.7 & \small 71.3 & \small 97.8 & \small 99.0 & \small .30  \\
\midrule
RNN-G-0.2       & \small 17 & \small 22.9 & \small 22.1 & \small 27.8 & \small 101.9 & \small 129.9 & \small 130.9 & \small .49 \\
\midrule
RNN-G-0.3       & \small 0 & \small 10.0 & \small 13.3 & \small 15.8 & \small 55.5 & \small 65.6 & \small 65.8 & \small .38 \\
\midrule
RNN-GM-0.5      & \small 14 & \small 18.7 & \small 20.0 & \small 25.1 & \small 94.5  & \small 127.5 & \small 127.7 & \small .38 \\
\midrule
RNN-GMB-0.5     & \small 28 & \small 67.2 & \small 25.2 & \small 27.4 & \small 78.8 & \small 95.9 & \small 99.6 & \small .23 \\
\midrule
LSTM-G-0.5      & \small 11 & \small 32.6 & \small 18.5 & \small 22.8 & \small 76.7 & \small 101.3 & \small 105.0 & \small .29 \\
\midrule
LSTM-G-0.2      & \small 8 & \small 14.8 & \small 19.9 & \small 24.6 & \small 77.8 & \small 98.8 & \small 100.7 & \small .31 \\
\midrule
LSTM-G-0.3      & \small 18 & \small 22.2 & \small 19.2 & \small 22.8 & \small 97.9  & \small 101.1 & \small 122.3 & \small .57 \\
\midrule
LSTM-GM-0.5     & \small 12 & \small 31.7 & \small 18.1 & \small 22.0 & \small 78.8 & \small 100.7 & \small 104.1 & \small .28 \\
\midrule
LSTM-GMB-0.5    & \small 8 & \small 23.0 & \small 19.3 & \small 24.8 & \small 78.9 & \small 104.4 & \small 107.7 & \small .30 \\
\midrule
GRU-G-0.5       & \small 15 & \small 44.0 & \small 18.3 & \small 23.5 & \small 94.0 & \small 119.5 & \small 131.7 & \small .35 \\
\midrule
GRU-G-0.2       & \small 6 & \small 14.8 & \small 17.9 & \small 22.4 & \small 60.9 & \small 82.3 & \small 83.5 & \small .27 \\
\midrule
GRU-G-0.3       & \small 3 & \small 13.9 & \small 16.8 & \small 19.9 & \small 68.6 & \small 81.8 & \small 82.1 & \small .46 \\
\midrule
GRU-GM-0.5      & \small 10 & \small 47.2 & \small 20.5 & \small 23.5 & \small 67.2 & \small 94.0 & \small 94.0 & \small .21 \\
\midrule
GRU-GMB-0.5     & \small 10 & \small 21.0 & \small 18.3 & \small 22.9 & \small 76.6 & \small 103.9 & \small 105.2 & \small .30 \\
\bottomrule
\end{tabular}}
\caption{Performance statistics of all assistant models when performing task as a solo pilot (values are averaged over 3$\times$30 sec. trials except \# crashes, which is summed). Columns from L--R: \# crashes, \% destabilizing actions, mean and SD distance from DOB, mean and SD angular velocity magnitude, RMS velocity, and mean deflection magnitude. Assistant model evaluations were conducted without noise added to deflection time or magnitude.}
\label{tab:assts}
\end{table*}

==> diff_table.tex <==
\begin{table*}[h!]
\centering
 \resizebox{\textwidth}{!}{
 \begin{tabular}{lcccccccc}
\toprule
\textbf{Assistant}        & \textbf{Crashes}$\downarrow$        & \textbf{\% destab.}$\downarrow$         & \textbf{$\mu\lvert\theta\rvert$ ($^\circ$)}$\downarrow$  & \textbf{$\sigma(\theta)$ ($^\circ$)}$\downarrow$   & \textbf{$\mu\lvert Mag\rvert_{vel}$ ($^\circ$/s)}$\downarrow$  & \textbf{$\sigma(\lvert Mag\rvert_{vel})$ ($^\circ$/s)}$\downarrow$ & \textbf{$vel$ RMS}$\downarrow$               & \textbf{$\mu\lvert d\rvert$}$\downarrow$   \\
\midrule
\small SAC      & \small \begin{tabular}[c]{@{}c@{}} 0 / -5 / -25\\ -8 / -25 / -12\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}2.2 / 4.9 / -18.3\\ -31.8 / -38.3 / -28.5\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}0.4 / 1.2 / -3.6\\ -2.0 / -7.6 -1.0\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}-0.9 / -6.6 / -7.9\\ -1.9 / -6.7 / 7.9\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}18.0 / -25.3 / -56.9\\ 27.0 / -37.7 / 7.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}18.4 / -36.6 / -54.3\\ 27.8 / -48.6 / 11.9\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}18.7 / -38.7 / -67.5\\ 24.4 / -42.2 / -6.9\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.1 / 0.0\\ 0.4 / -0.1 / 0.3\end{tabular}  \\ \midrule
\small SAC-BC   & \small \begin{tabular}[c]{@{}c@{}}1 / -1 / -22\\ 0 / -20 / -3\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.8 / -2.0 / -22.6\\ -27.5 / -34.1 / -26.3\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}2.1 / 0.1 / 7.8\\ -2.3 / -7.6 / -1.3\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}1.0 / 1.1 / 6.1\\ -1.7 / -5.6 / 8.8\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}14.1 / -5.4 / -52.6\\ 24.6 / -38.5 / 16.3\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}16.7 / -8.8 / -46.5\\ 35.3 / -47.0 / 27.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}17.0 / -9.6 / -58.9\\ 31.4 / -42.4 / 9.5\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.1 / -0.0 / -0.0\\ 0.2 / -0.3 / 0.1\end{tabular}   \\ \midrule
\small SAC-AIRL & \small \begin{tabular}[c]{@{}c@{}}-2 / -7 / -17\\ -15 / -33 / -12\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}1.9 / -3.8 / -14.4\\ -36.8 / -41.5 / -28.5\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}1.9 / -0.1 / 5.4\\ -0.5 / -6.1 / 0.9\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}0.9 / -7.7 / -0.3\\ -6.8 / -10.9 / 9.1\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}-9.8 / -38.7 / -62.8\\ -22.5 / -66.6 / -8.7\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}-11.0 / -49.8 / -61.0\\ -26.1 / -71.7 / -19\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}-11.2 / -53.5 / -71.2\\ -29.9 / -72.9 / -20.3\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}0.1 / -0.1 / -0.0\\ 0.2 / -0.2 / 0.2\end{tabular} \\ \midrule
\small DDPG     & \small \begin{tabular}[c]{@{}c@{}}1 / -2 / -21\\ -11 / -23 / -12\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}2.3 / 3.7 / -17.3\\ -36.4 / -36.4 / -25.1\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}2.4 / -2.4 / -2.2\\ 2.6 / -7.5 / -1.0\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}2.1 / -3.1 / -3.4\\ 3.5 / -3.6 / 9.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}25.3 / -11.0 / -43.1\\ 47.4 / -34.1 / 5.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}22.4 / -19.7 / -38.2\\ 47.3 / -36.6 / 7.24\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}24.6 / -21.2 / -51.0\\ 43.5 / -38.6 / -12.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.1 / 0.1\\ 0.6 / -0.1 / 0.3\end{tabular}  \\ \midrule
\small DDPG-BC  & \small \begin{tabular}[c]{@{}c@{}}1 / 2 / -19\\ -6 / -20 / -8\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.8 / -0.5 / -19.1\\ -31.3 / -30.4 / -27.9\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}4.9 / 4.2 / 1.5\\ -2.7 / -8.6 / 4.4\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}4.5 / 5.3 / -9.8\\ -2.0 / -7.5 / 13.6\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}18.1 / 7.4 / -56.5\\ 4.5. / -34.4 / 11.6\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}17.3 / 1.3 / -51.5\\ 3.4 / -37.0 / 16.3\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}18.1 / -0.8 / -61.4\\ 2.9 / -37.1 / -1.7\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.1 / 0.0 / -0.1\\ 0.1 / -0.2 / 0.1\end{tabular} \\ \midrule
\small MLP-G-0    & \small \begin{tabular}[c]{@{}c@{}}-2 / 6 / -12\\ 5 / -10 / -9\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}1.6 / 13.6 / -8.1\\ -14.6 / -20.8 / -25.0\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}4.3 / 2.2 / 0.5\\ 1.1 / -3.1 / 4.5\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}2.8 / -0.4 / 0.1\\ 1.9 / 0.1 / 13.9\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}12.3 / -4.3 / -43.5\\ 35.8 / -3.6 / 11.2\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}11.9 / -19.0 / -36.7\\ 50.3 / -9.9 / 22.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}10.4 / -8.0 / -48.0\\ 46.5 / -5.0 / 2.6\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular} \\ \midrule
\small MLP-G-0.5    & \small \begin{tabular}[c]{@{}c@{}}6 / 8 / -8\\ 8 / -20 / 8\end{tabular}        & \small \begin{tabular}[c]{@{}c@{}}11.2 / 14.2 / -1.6\\ -6.4 / -27.7 / -8.1\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}2.0 / 5.6 / 1.3\\ 0.3 / -4.4 / -0.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}0.1 / 0.9 / -3.7\\ 0.3 / -2.4 / 9.4\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}19.2 / -0.5 / -39.0\\ 39.2 / -32.5 / 39.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}23.9 / -18.5 / -32.3\\ 45.6 / -35.3 / 53.9\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}26.0 / -5.8 / -40.2\\ 47.5 / -36.7 / 37.4\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.1 / -0.0 / -0.1\\ 0.2 / -0.1 / 0.2\end{tabular} \\ \midrule
\small MLP-G-0.2    & \small \begin{tabular}[c]{@{}c@{}}7 / 12 / -7\\ 5 / -14 / 4\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}11.5 / 20.5 / -4.1\\ -10.7 / -22.3 / -6.1\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}2.9 / 1.9 / 0.4\\ 0.8 / -6.5 / 1.1\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}2.2 / -1.1 / -0.1\\ 1.6 / -3.8 / 9.3\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}26.3 / 3.0 / -30.0\\ 34.5 / -16.8 / 22.7\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}33.9 / -17.5 / -22.6\\ 45.2 / -29.1 / 35.3\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}32.5 / 2.6 / -33.3\\ 46.3 / -15.6 / 18.3\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.1 / -0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular} \\ \midrule
\small MLP-G-0.3    & \small \begin{tabular}[c]{@{}c@{}}3 / 14 / -7\\ 3 / -14 / 3\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}3.8 / 25.2 / -7.0\\ -17.5 / -21.8 / -18.5\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}4.7 / 0.7 / 2.3\\ -0.7 / -6.7 / 2.0\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}4.1 / 0.8 / 1.6\\ 0.5 / -3.2 / 12.0\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}27.9 / 14.7 / -41.4\\ 33.5 / -16.0 / 33.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}31.1 / -18.1 / -39.2\\ 41.7 / -24.9 / 45.2\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}32.9 / 12.1 / -48.6\\ 40.1 / -17.9 / 25.8\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.1\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small MLP-GM-0   & \small \begin{tabular}[c]{@{}c@{}}-1 / 3 / -12\\ 1 / -18 / -1\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}2.0 / 8.3 / -10.4\\ -17.4 / -27.6 / -15.3\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}3.4 / 3.1 / -1.6\\ 0.5 / -6.1 / 4.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}2.9 / 1.5 / -2.9\\ 1.3 / -2.5 / 12.8\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}16.4 / 7.7 / -45.8\\ 31.3 / -17.0 / 18.7\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}22.2 / -2.2 / -38.5\\ 40.7 / -20.4 / 21.4\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}22.3 / 2.7 / -47.7\\ 37.5 / -19.4 / 5.5\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small MLP-GMB-0  & \small \begin{tabular}[c]{@{}c@{}}-2 / 4 / -11\\ -1 / -18 / -4\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}-0.5 / 7.0 / -8.8\\ -21.6 / -29.7 / -21.5\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}2.4 / 3.1 / 2.2\\ 2.1 / -6.8 / 4.0\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}2.2 / 2.8 / -1.7\\ 0.8 / -2.5 / 12.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}18.8 / 7.0 / -43.2\\ 31.4 / -15.5 / 12.2\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}25.0 / -5.1 / -36.3\\ 41.5 / -20.3 / 22.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}24.5 / 1.3 / -48.0\\ 38.7 / -18.6 / 3.8\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small RNN-G-0.5    & \small \begin{tabular}[c]{@{}c@{}}7 / 8 / -2\\ 6 / -10 / 1\end{tabular}        & \small \begin{tabular}[c]{@{}c@{}}11.6 / 18.2 / -3.4\\ -6.4 / -18.4 / -9.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.3 / 4.2 / 1.7\\ -1.1 / -8.5 / -0.2\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}2.8 / 0.8 / 3.3\\ -0.8 / -4.3 / 8.7\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}24.5 / 2.8 / -22.0\\ 30.1 / -2.5 / 26.0\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}30.5 / -13.6 / -11.5\\ 45.9 / -5.9 / 37.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}29.6 / 1.1 / -23.6\\ 46.6 / 0.8 / 25.0\end{tabular}        & \small \begin{tabular}[c]{@{}c@{}}0.1 / -0.0 / -0.0\\ 0.2 / -0.1 / 0.2\end{tabular} \\ \midrule
\small RNN-G-0.2    & \small \begin{tabular}[c]{@{}c@{}}5 / 11 / -4\\ 6 / -15 / 0\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}7.5 / 18.6 / -3.4\\ -15.7 / -23.1 / -8.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}4.4 / 2.6 / -1.0\\ 0.1 / -7.4 / 0.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.4 / 1.8 / -2.1\\ 0.3 / -4.0 / 9.8\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}24.8 / 13.9 / -24.3\\ 44.8 / -16.2 / 20.4\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}37.1 / -10.0 / -15.2\\ 53.9 / -12.8 / 35.2\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}37.6 / 10.8 / -24.6\\ 51.4 / -14.5 / 19.4\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.1 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small RNN-G-0.3    & \small \begin{tabular}[c]{@{}c@{}}2 / 14 / -10\\ -2 / -18 / -5\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}4.0 / 19.6 / -10.7\\ -21.5 / -22.2 / -20.3\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}3.7 / 0.5 / 2.5\\ -0.1 / -6.5 / 0.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}.7 / -0.3 / 1.9\\ 0.9 / -4.1 / 10.2\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}15.9 / 13.0 / -32.6\\ 29.3 / -24.2 / 18.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}23.4 / -22.7 / -25.0\\ 37.7 / -30.5 / 28.7\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}25.0 / 7.1 / -38.0\\ 35.0 / -24.4 / 13.8\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.2 / -0.2 / 0.2\end{tabular} \\ \midrule
\small RNN-GM-0.5   & \small \begin{tabular}[c]{@{}c@{}}10 / 14 / -8\\ 6 / -19 / 0\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}13.2 / 22.9 / -6.7\\ -9.2 / -26.7 / -8.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}1.8 / 1.9 / 1.2\\ 0.4 / -7.5 / 2.4\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}1.8 / -0.2 / 0.5\\ 1.2 / -4.6 / 11.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}27.8 / 13.8 / -32.7\\ 44.9 / -21.4 / 21.0\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}41.3 / -18.9 / -22.3\\ 62.7 / -22.4 / 34.6\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}41.7 / 11.0 / -34.4\\ 58.6 / -20.4 / 18.1\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.1 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small RNN-GMB-0.5  & \small \begin{tabular}[c]{@{}c@{}}7 / 4 / -6\\ 6 / -10 / 3\end{tabular}        & \small \begin{tabular}[c]{@{}c@{}}10.2 / 14.3 / -6.6\\ -7.3 / -13.9 / -9.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}4.7 / 3.0 / 1.7\\ 0.6 / -7.0 / 3.6\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}3.8 / 3.4 / -1.3\\ 0.1 / -4.4 / 13.4\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}29.3 / 3.6 / -26.8\\ 33.6 / -4.2 / 34.8\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}41.5 / -4.8 / -23.0\\ 48.7 / -12.8 / 50.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}41.4 / 3.6 / -28.6\\ 47.5 / 0.6 / 31.5\end{tabular}        & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small LSTM-G-0.5   & \small \begin{tabular}[c]{@{}c@{}}4 / 8 / -10\\ 4 / -16 / 1\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}7.7 / 18.6 / -7.5\\ -7.9 / -19.7 / -10.8\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}2.3 / 2.1 / -1.5\\ -1.3 / -7.8 / 2.9\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}1.5 / 0.3 / -0.7\\ -0.7 / -5.3 / 13.2\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}30.9 / 10.0 / -26.6\\ 33.2 / -13.9 / 30.9\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}37.0 / -19.3 / -20.3\\ 49.5 / -23.7 / 46.3\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}38.2 / 4.3 / -29.8\\ 46.7 / -16.0 / 28.1\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.2 / -0.1 / 0.2\end{tabular} \\ \midrule
\small LSTM-G-0.2   & \small \begin{tabular}[c]{@{}c@{}}3 / 14 / -7\\ 4 / -13 / 1\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}8.0 / 23.5 / -1.6\\ -11.0 / -20.5 / -8.8\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.6 / -0.2 / 0.9\\ 1.7 / -7.3 / 3.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}2.8 / 0.6 / 1.5\\ 2.7 / -4.0 / 12.6\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}25.4 / 15.6 / -33.7\\ 32.9 / -13.2 / 27.4\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}33.1 / -15.2 / -22.5\\ 43.8 / -24.4 / 43.6\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}34.6 / 15.2 / -33.2\\ 41.5 / -14.2 / 24.8\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.2 / -0.1 / 0.2\end{tabular} \\ \midrule
\small LSTM-G-0.3   & \small \begin{tabular}[c]{@{}c@{}}1 / 1 / -16\\ 0 / -19 / -2\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}2.6 / 5.2 / -13.6\\ -21.7 / -24.7 / -18.1\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}5.7 / 1.2 / 2.8\\ 0.7 / -5.7 / 1.9\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}4.5 / -0.1 / 1.5\\ 0.4 / -2.8 / 11.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}12.2 / -8.4 / -40.2\\ 30.5 / -30.1 / 23.5\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}11.2 / -18.5 / -36.6\\ 30.5 / -45.3 / 32.0\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}12.2 / -15.1 / -48.1\\ 34.6 / -30.4 / 15.5\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.3 / -0.2 / 0.2\end{tabular} \\ \midrule
\small LSTM-GM-0.5  & \small \begin{tabular}[c]{@{}c@{}}5 / 5 / -15\\ 5 / -21 / -3\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}7.0 / 10.7 / -10.0\\ -7.0 / -29.1 / -15.1\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}4.5 / 1.3 / 2.1\\ -2.0 / -7.5 / 0.9\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}4.5 / -1.1 / -1.7\\ -0.7 / -4.4 / 10.1\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}27.9 / -0.8 / -38.7\\ 41.1 / -15.7 / 23.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}38.6 / -23.1 / -31.4\\ 55.6 / -16.3 / 32.0\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}37.4 / -7.8 / -41.4\\ 54.4 / -17.3 / 18.2\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.2 / -0.1 / 0.2\end{tabular} \\ \midrule
\small LSTM-GMB-0.5 & \small \begin{tabular}[c]{@{}c@{}}9 / 13 / -11\\ 6 / -15 / -3\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}12.7 / 25.4 / -9.2\\ -4.5 / -19.1 / -11.2\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}1.1 / 0.9 / 0.8\\ -0.4 / -4.8 / 4.4\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}1.5 / 0.1 / 1.1\\ 0.9 / -1.4 / 10.6\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}24.8 / 13.8 / -29.2\\ 40.4 / -11.6 / 19.0\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}27.6 / -15.7 / -20.7\\ 54.1 / -16.6 / 36.3\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}31.4 / 12.3 / -31.9\\ 51.8 / -12.3 / 18.8\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.1 / -0.0 / -0.0\\ 0.2 / -0.1 / 0.2\end{tabular} \\ \midrule
\small GRU-G-0.5    & \small \begin{tabular}[c]{@{}c@{}}5 / 4 / -10\\ 3 / -15 / -4\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}8.0 / 11.9 / -3.0\\ -7.7 / -18.0 / -17.2\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.0 / 2.1 / -1.9\\ 0.3 / -6.1 / 0.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.4 / 1.3 / -2.7\\ 1.4 / -2.6 / 9.1\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}30.0 / 8.2 / -36.4\\ 43.2 / -3.1 / 24.0\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}41.3 / -11.1 / -25.8\\ 59.3 / -8.9 / 39.7\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}44.3 / 2.1 / -37.5\\ 59.1 / -0.6 / 22.8\end{tabular}       & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small GRU-G-0.2    & \small \begin{tabular}[c]{@{}c@{}}7 / 6 / -8\\ 2 / -14 / 5\end{tabular}        & \small \begin{tabular}[c]{@{}c@{}}5.8 / 8.7 / -7.5\\ -15.3 / -24.9 / -11.9\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.1 / 4.0 / 0.1\\ -1.2 / -6.9 / 0.8\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}3.6 / 2.8 / 0.9\\ -0.5 / -3.1 / 10.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}25.9 / 5.5 / -32.2\\ 40.8 / -7.0 / 36.4\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}33.5 / -11.3 / -19.9\\ 62.1 / -18.3 / 42.5\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}33.5 / -1.0 / -32.5\\ 58.3 / -7.8 / 30.8\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small GRU-G-0.3    & \small \begin{tabular}[c]{@{}c@{}}3 / 3 / -18\\ -3 / -16 / -3\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}6.6 / 11.0 / -15.1\\ -26.0 / -21.3 / -16.2\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}5.6 / 3.5 / 6.2\\ 2.4 / -5.9 / 1.2\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}3.6 / -1.0 / 5.9\\ 3.5 / -2.4 / 9.9\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}13.8 / -13.2 / -44.5\\ 33.3 / -24.7 / 17.7\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}12.8 / -26.6 / -35.7\\ 42.4 / -30.1 / 29.3\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}14.2 / -18.6 / -48.8\\ 38.3 / -24.9 / 13.0\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / 0.0\\ 0.3 / -0.2 / 0.2\end{tabular}  \\ \midrule
\small GRU-GM-0.5   & \small \begin{tabular}[c]{@{}c@{}}7 / 8 / -10\\ 4 / -19 / -1\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}10.5 / 16.3 / -4.2\\ -10.9 / -27.7 / -12.6\end{tabular} & \small \begin{tabular}[c]{@{}c@{}}5.3 / -0.3 / -0.6\\ 0.4 / -6.6 / 1.9\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}4.2 / 1.4 / -0.8\\ 1.0 / -2.9 / 11.7\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}30.7 / 13.4 / -31.7\\ 40.7 / -17.9 / 24.9\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}37.8 / -8.8 / -19.6\\ 54.7 / -29.0 / 41.0\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}39.2 / 12.0 / -30.8\\ 51.3 / -22.4 / 21.4\end{tabular}     & \small \begin{tabular}[c]{@{}c@{}}0.2 / 0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular}  \\ \midrule
\small GRU-GMB-0.5  & \small \begin{tabular}[c]{@{}c@{}}8 / 13 / -11\\ 2 / -16 / 1\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}10.3 / 25.5 / -7.3\\ -11.0 / -21.7 / -7.6\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}1.7 / 2.1 / 2.0\\ 0.1 / -5.0 / 0.0\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}1.1 / 0.2 / 2.5\\ 1.3 / -3.0 / 10.0\end{tabular}    & \small \begin{tabular}[c]{@{}c@{}}30.9 / 12.4 / -34.8\\ 42.0 / -11.4 / 32.6\end{tabular}   & \small \begin{tabular}[c]{@{}c@{}}41.0 / -19.6 / -24.0\\ 56.5 / -18.7 / 51.1\end{tabular}  & \small \begin{tabular}[c]{@{}c@{}}40.9 / 11.1 / -34.7\\ 55.6 / -9.4 / 32.2\end{tabular}      & \small \begin{tabular}[c]{@{}c@{}}0.2 / -0.0 / -0.0\\ 0.3 / -0.1 / 0.2\end{tabular} \\
\bottomrule
\end{tabular}}
\caption{Differences in performance with and without assistance (e.g., {\it 0} means no change in that metric). In each cell, top line refers to MARS pilot models and bottom to VIP pilot models, and slashes separate Good, Medium, and Bad pilot models.  In the Assistant column, G/M/B denotes the proficiency of the assistant training data, decimals denote window size (for window size 0.3s, future prediction was always 0.1s; for all other window sizes, the next step [0.0s] was predicted).}
\label{tab:diff}
\end{table*}

==> model_comparison.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{llll}
\toprule
{\bf Type}      & {\bf Input}           & {\bf Prediction}      & {\bf \# params}   \\
\midrule
\small SAC      & \small Current step   & \small Next step      & \small 268.0K$^\dag$ \\ 
\midrule
\small DDPG     & \small Current step   & \small Next step      & \small 244.8K$^\dag$ \\ 
\midrule
\small MLP      & \small Current step   & \small Next step      & \small 20.7.0K    \\ 
                & \small Past 0.2s      & \small Next step      & \small 23.7.0K    \\ 
                & \small Past 0.3s      & \small 0.1s future    & \small 25.2.0K    \\ 
                & \small Past 0.5s      & \small Next step      & \small 28.2.0K      \\ 
\midrule
\small RNN      & \small Past 0.2s      & \small Next step      & \small 101.0K     \\ 
                & \small Past 0.3s      & \small 0.1s future    & \small 101.0K     \\ 
                & \small Past 0.5s      & \small Next step      & \small 101.0K     \\ 
\midrule
\small LSTM     & \small Past 0.2s      & \small Next step      & \small 314.0K     \\ 
                & \small Past 0.3s      & \small 0.1s future    & \small 314.0K     \\ 
                & \small Past 0.5s      & \small Next step      & \small 314.0K     \\ 
\midrule
\small GRU      & \small Past 0.2s      & \small Next step      & \small 243.0K     \\ 
                & \small Past 0.3s      & \small 0.1s future    & \small 243.0K     \\ 
                & \small Past 0.5s      & \small Next step      & \small 243.0K     \\
%\midrule
%\small Informer & \small Past 0.3s      & \small 0.1s future    & \small 3.4G       \\ 
\bottomrule
\end{tabular}
\caption{Model statistics.}
\label{tab:model-comparison}
\begin{tablenotes}
      \footnotesize
      \item $^\dag$Sum over all actor and critic networks.
\end{tablenotes}
\end{table}
